Auditing Retrieval-Augmented LLM Hypotheses for Longitudinal Cell Painting Morphology

High-content morphological profiling (Cell Painting) yields sensitive, high-dimensional signatures of cellular state, but translating longitudinal morphology trajectories into interpretable biology remains difficult, especially for weak, chronic perturbations such as low-dose-rate ionizing radiation. Large language models (LLMs) can synthesize heterogeneous evidence into biological narratives, yet their scientific use requires quantitative auditing. We present an evaluation-first, retrieval-augmented interpretation framework for longitudinal Cell Painting morphology, applied to a 9-week RPE-1 time course across five dose rates (0.003--6.0 mGy/hr). Week-matched treated-control morphology deltas are combined with retrieved perturbation neighbors, pathway context, and literature evidence through stable evidence identifiers, enabling an LLM to generate structured, evidence-linked hypotheses that are hierarchically summarized while preserving provenance. We introduce two quantitative auditing tests: V1 citation validity, which verifies that cited evidence identifiers exist in the prompt, and V2 proxy-based morphology compatibility, which evaluates consistency between predicted biological processes and the most altered morphology features. In our experiments, V1 detected no invalid evidence references, while V2 showed meaningful morphology compatibility that increased with perturbation strength and was positively associated with an independent morphology drift summary. The framework produces auditable, falsifiable biological hypotheses, including an adaptive phenotype involving metabolic reprogramming and proteostatic stress at lower dose rates (0.003--0.3 mGy/hr). Current limitations include proxy-based evaluation and the lack of ground-truth mechanism labels.

==> TableS1_drift_correlation_summary.tex <==
\begin{tabular}{@{} l c c c @{}}
\toprule
\textbf{Comparison} & $\boldsymbol{n}$ & \textbf{Pearson} $\boldsymbol{r}$ \textbf{(95\% CI)} & \textbf{Spearman} $\boldsymbol{\rho}$ \textbf{(95\% CI)} \\
\midrule
Step~4 AUC vs. dose\_time mean Hit@10 & 5 & $0.625$ [$-$0.439, 1.000] & $0.700$ [$-$0.875, 1.000] \\
\addlinespace
Step~4 mean drift vs. dose\_time mean Hit@10 & 5 & $0.661$ [$-$0.363, 1.000] & $0.700$ [$-$0.875, 1.000] \\
\addlinespace
Step~4 slope vs. global mean Hit@10 & 5 & $0.000$ [$-$1.000, 1.000] & $-$0.300 [$-$1.000, 1.000] \\
\bottomrule
\multicolumn{4}{@{}l}{\footnotesize \textit{Note:} Bootstrap $n_{\mathrm{boot}}=10{,}000$, seed=42, CI=percentile 95\%.}
\end{tabular}
